SafaRi:Adaptive Sequence Transformer for Weakly Supervised Referring Expression Segmentation

Referring Expression Segmentation (RES) aims to provide a segmentation mask of the target object in an image referred to by the text (i.e., referring expression). Existing methods require large-scale mask annotations. Moreover, such approaches do not generalize well to unseen/zero-shot scenarios. To address the aforementioned issues, we propose a weakly-supervised bootstrapping architecture for RES with several new algorithmic innovations. To the best of our knowledge, ours is the first approach that considers only a fraction of both mask and box annotations (shown in Figure 1 and Table 1) for training. To enable principled training of models in such low-annotation settings, improve image-text region-level alignment, and further enhance spatial localization of the target object in the image, we propose Cross-modal Fusion with Attention Consistency module. For automatic pseudo-labeling of unlabeled samples, we introduce a novel Mask Validity Filtering routine based on a spatially aware zero-shot proposal scoring approach. Extensive experiments show that with just 30% annotations, our model SafaRi achieves 59.31 and 48.26 mIoUs as compared to 58.93 and 48.19 mIoUs obtained by the fully-supervised SOTA method SeqTR respectively on RefCOCO+@testA and RefCOCO+testB datasets. SafaRi also outperforms SeqTR by 11.7% (on RefCOCO+testA) and 19.6% (on RefCOCO+testB) in a fully-supervised setting and demonstrates strong generalization capabilities in unseen/zero-shot tasks.

==> graphs/data_label_rates.tex <==
\begin{tikzpicture}
	\begin{axis} [
		axis x line*=bottom,
		axis y line*=left,
		legend pos=north east,
		ymin=60, ymax=75,
		xmin=10.0, xmax=100.0,
		xticklabel={\pgfmathparse{\tick}\pgfmathprintnumber{\pgfmathresult}},
		xtick={10.0,20.0,30.0,50.0,70.0,100.0},
		ytick={60,65,70,75},
        xlabel={label-rate},
        ylabel={mIoU},
		width=\linewidth,
		legend style={cells={align=left}},
		label style={font=\normalsize},
		tick label style={font=\normalsize},
		legend style={draw=none,at={(0.35,0.25)},anchor=west},
		]

        \addplot[mark=*,mark options={scale=1.0, fill=Dark},style={thick},Dark] plot coordinates {
			(10.0, 64.02)
            (20.0, 65.88)
			(30.0, 67.04)
            (50.0, 70.59)
            (70.0, 72.53)
			(100.0, 73.35)
		};
        \addlegendentry{Ours}

		\addplot[dashed,gray] plot coordinates {
			(0, 67.26)
			(100, 67.26)
		};
        \addlegendentry{SeqTR \cite{zhu2022seqtr}}
		% \addplot[mark=asterisk,color_ao,mark options={scale=2,thick},only marks] plot coordinates {
		% 	(1, 67.26)
		% };
		\label{pgf:ek100_map}
	\end{axis}
\end{tikzpicture}



==> graphs/plot_1.tex <==
\begin{figure}[!b]
\vspace{-5mm}
	\centering
	% \begin{subfigure}[b]{\linewidth}
	% 	\centering
	% 	\begin{tikzpicture}
	% 		\begin{customlegend}
	% 			[
	% 			legend columns=3, legend style={column sep=0.2ex},
	% 			legend entries={\small{WSRES(30\%)},\small{WSRES(10\%)},\small{SeqTR~\cite{zhu2022seqtr}}
	% 			}]
	% 			\addlegendimage{mark=triangle,style={thick},Dark}
	% 			\addlegendimage{mark=o,style={thick},gray}
	% 			\addlegendimage{mark=asterisk,color_ao,mark options={scale=2,thick},only marks}
	% 		\end{customlegend}
	% 	\end{tikzpicture}
	% \end{subfigure}

    % \vspace{0.5em}
    \hspace{-0.55em}
	\begin{subfigure}[b]{0.495\linewidth}
		\resizebox{1.0\textwidth}{!}{
			\input{graphs/data_gamma}%
		}
		\caption{mIoU vs runs.}
        \label{fig:runs}
	\end{subfigure}
 \hspace{-0em}
	\begin{subfigure}[b]{0.495\linewidth}
		\resizebox{1.0\textwidth}{!}{
			\input{graphs/data_lambda}%
		}
		\caption{mIoU vs $\lambda$.}
        \label{fig:lambda}
	\end{subfigure}
 %    \begin{subfigure}[b]{0.8\linewidth}
	% 	\resizebox{\textwidth}{0.5\textwidth}{
	% 		\input{graphs/data_lambda}%
	% 	}
	% 	\caption{mIoU vs $\lambda$.}
	% \end{subfigure}
	\caption{\textbf{Impact of $\gamma$-scheduling under different initial values ($\gamma_{0}$) and AMCR balancing factor ($\lambda$)} on model performance evaluated on RefCOCO@val set under 30\% and 10\% mask labels.}
\end{figure}

==> graphs/plot_2.tex <==
\begin{figure}[!b]
	\centering
	% \begin{subfigure}[b]{\linewidth}
	% 	\centering
	% 	\begin{tikzpicture}
	% 		\begin{customlegend}
	% 			[
	% 			legend columns=3, legend style={column sep=0.2ex},
	% 			legend entries={\small{WSRES(30\%)},\small{WSRES(10\%)},\small{SeqTR~\cite{zhu2022seqtr}}
	% 			}]
	% 			\addlegendimage{mark=triangle,style={thick},Dark}
	% 			\addlegendimage{mark=o,style={thick},gray}
	% 			\addlegendimage{mark=asterisk,color_ao,mark options={scale=2,thick},only marks}
	% 		\end{customlegend}
	% 	\end{tikzpicture}
	% \end{subfigure}

    % \vspace{0.5em}
	
    \resizebox{0.4\textwidth}{!}{
        \input{graphs/data_label_rates}%
    }
    \caption{mIoU vs label-rates.}
    \label{fig:miou_label_rates}

\end{figure}
